Improving Network Robustness against Adversarial Attacks with Compact Convolution

Though Convolutional Neural Networks (CNNs) have surpassed human-level performance on tasks such as object classification and face verification, they can easily be fooled by adversarial attacks. These attacks add a small perturbation to the input image that causes the network to misclassify the sample. In this paper, we focus on neutralizing adversarial attacks by compact feature learning. In particular, we show that learning features in a closed and bounded space improves the robustness of the network. We explore the effect of L2-Softmax Loss, that enforces compactness in the learned features, thus resulting in enhanced robustness to adversarial perturbations. Additionally, we propose compact convolution, a novel method of convolution that when incorporated in conventional CNNs improves their robustness. Compact convolution ensures feature compactness at every layer such that they are bounded and close to each other. Extensive experiments show that Compact Convolutional Networks (CCNs) neutralize multiple types of attacks, and perform better than existing methods in defending adversarial attacks, without incurring any additional training overhead compared to CNNs.

==> loss.tex <==
\section{Robust Loss Functions}
\label{sec:loss_functions}

In this section, we provide an overview of CenterLoss~\cite{wen2016discriminative} and $L_{2}$-Softmax Loss~\cite{ranjan2017l2}, which enhance the network's robustness to adversarial attacks by following the principles of \textit{centrality} and \textit{compactness}.

\subsection{CenterLoss}
\label{sec:CenterLoss}
The CenterLoss was proposed by Wen et al.~\cite{wen2016discriminative} for the task of discriminative face verification. It simultaneously learns a center for deep features of each class and penalizes the distances between the deep features and their corresponding class centers. The structure of the loss function is shown in (\ref{eq:centerloss}):

\begin{equation}
\small
\label{eq:centerloss}
L_{C} = -\sum_{i=1}^{m} \log \frac{e^{W_{y_{i}}^{T}\mathbf{x}_{i} + b_{y_{i}}}}{\sum_{j=1}^{n} e^{W_{j}^{T}\mathbf{x}_{i} + b_{j}}} + \lambda \frac{1}{2} \sum_{i=1}^{m} \|\mathbf{x}_{i} - \mathbf{c}_{y_{i}}\|_{2}^{2},
\end{equation}

where $\mathbf{x}_{i}$ is the $i^{th}$ deep feature and $c_{y_{i}}$ is the center for the class label $y_{i}$, $W_{j}$ is the weight and $b_{j}$ is the bias corresponding to the class $j$, and $m$, $n$ are the batch-size and number of classes respectively. The first term is the typical softmax loss that encourages inter-class separability. The second term is the distance penalty that ensures the closeness of intra-class deep features. The hyper-parameter $\lambda$ controls the trade-off between intra-class and inter-class variability. 

We use CenterLoss as a defense to adversarial attacks owing to its \textit{centrality} property. Experimental results suggest that CenterLoss improves network robustness compared to traditional softmax loss.
